On the Effectiveness of Hybrid Mutual Information Estimation

Estimating the mutual information from samples from a joint distribution is a challenging problem in both science and engineering. In this work, we realize a variational bound that generalizes both discriminative and generative approaches. Using this bound, we propose a hybrid method to mitigate their respective shortcomings. Further, we propose Predictive Quantization (PQ): a simple generative method that can be easily combined with discriminative estimators for minimal computational overhead. Our propositions yield a tighter bound on the information thanks to the reduced variance of the estimator. We test our methods on a challenging task of correlated high-dimensional Gaussian distributions and a stochastic process involving a system of free particles subjected to a fixed energy landscape. Empirical results show that hybrid methods consistently improved mutual information estimates when compared to the corresponding discriminative counterpart.

==> figures/graphical_model.tex <==
\begin{figure}[h]
\centering
\begin{tikzpicture}[latent/.style={circle, draw, minimum size=0.5cm, text width=0.5cm, align=center, font=\relsize{-2}}]
      \node[latent] (u_p) {$u_{k-1}$}; %
      \node[latent, right=of u_p] (u_k) {$u_k$}; % 
      \node[latent, right=of u_k] (u_f) {$u_{k + 1}$}; % 
      
      \node[latent, below=of u_p] (z_p) {$z_{k-1}$}; %
      \node[latent, below=of u_k] (z_k) {$z_k$}; % 
      \node[latent, below=of u_f] (z_f) {$z_{k + 1}$}; % 
      
      \node[left=.1cm of z_p] (z_ld) {$\dots$}; % 
      \node[right=.1cm of z_f] (z_rd) {$\dots$}; % 
      
      \edge{u_p}{z_p}; %
      \edge{u_k}{z_k}; %
      \edge{u_f}{z_f}; %
      \edge{z_k}{z_p}; %
      \edge{z_f}{z_k}; %
\end{tikzpicture}
\caption{\dr{Adjust styling}}
\label{fig:graphical_model}
\end{figure}

==> tables/comparison.tex <==
\begin{table}[!t]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
         & \multicolumn{2}{c|}{ Unnormalized } & \multicolumn{4}{c|}{ Normalized }\\\cline{2-7} 
         &  $f_\theta(\vx,\vy)$ & $f_\theta(\vx,\vy)-C(\vx)$ & $\log\left(\left|\frac{\partial g_\vx(\vy)}{\partial \vy}\right|+\left|\frac{\partial g_\vx(\vy)}{\partial \vy}\right|\right)$ & $\log\left|\frac{\partial g_\vx(\vy)}{\partial \vy}\right|$ & $\log\left|\frac{\partial g(\vx,\vy)}{\partial\vx\partial\vy}\right|$ & 0\\\hline
         $r_\phi(x,y)$ & & & & & & \\
         $p(x|y) r_\phi(y)$ & & & & & & \\
         $p(x)r_\phi(y|x)$ & - & * & * & BA+Flow & * & BA\\
         $p(x)p(y)$ & MINE & DV & * & * & * & 0 \\\hline
    \end{tabular}
    \caption{TODO:write caption and check if we need to remove/add columns or rows}
    \label{tab:my_label}
\end{table}

==> tables/t_comparison.tex <==
\begin{table}[t!]
\begin{tabular}{l|l|l|l}%|l|l}
Model & Proposal & Energy & Baseline \\\hline%& Bias                                       & Variance                              \\\hline
BA \citep{barber2003im} & $p(\rvz_1)r_\theta(\rvz_2|\rvz_1)$                                                     & $k$ & $k$                                                                                   \\%& $\KL(p||r_{\hat\theta})$                            & small                                 \\
InfoNCE \citep{oord2018representation} & $p(\rvz_1)p(\rvz_2)$ & $f_\phi^{\vz_1}(\vz_1)^T f_\phi^{\vz_2}(\vz_2)-\log\left(\frac{1}{K}\sum_{i=1}^K e^{f_\phi^{\vz_1}(\vz_1^{(i)})^T f_\phi^{\vz_2}(\vz_2)}\right)$ & $0$                                                                                 \\% & $I(\rvx;\rvy)-\log K$        & small                                 \\
NWJ \citep{nguyen2010estimating} & $p(\rvz_1)p(\rvz_2)$ & $f_\phi(\vz_1,\vz_2)$ & $1$                                               \\%& $\KL(p||q_{\hat\phi})$                                             & $e^{I(\rvx;\rvy)}-1$ \\
TUBA \citep{poole2019variational} & $p(\rvz_1)p(\rvz_2)$ & $f_\phi(\vz_1,\vz_2)$ & $a_\psi(\vz_2)$                                              \\% & $\KL(p||q_{\hat\phi})$                                            & $e^{I(\rvx;\rvy)}-1$ \\
FLO \citep{TODO} & $p(\rvz_1)p(\rvz_2)$ & $f_\phi(\vz_1,\vz_2)$ & $a_\psi(\vz_1,\vz_2)+f_\phi(\vz_1,\vz_2)$ \\
\textbf{VP}[ours] & $p(\rvz_1)r_\theta(\rvz_2|\rvz_1)$ & $f_\phi(\vz_1,\vz_2)$                                       & $a_\psi(\vz_1,\vz_2)$\\%& $\KL(p||q_{\hat\theta\hat\phi})$                                             & $e^{\KL(p||r_{\hat\theta})}-1$
\textbf{AP}[ours] & $p(\rvz_1)\E[p(\rvz_2|\va)]$ & $f_\phi(\vz_1,\vz_2)$   & $a_\psi(\vz_1,\vz_2)$                                    \\%& $\KL(p||q_{\hat\theta\hat\phi})$                                             & $e^{\KL(p||r_{\hat\theta})}-1$
\end{tabular}
\caption{Comparison of choices of proposal distribution $r(\rvz_1,\rvz_2)$ and energy transformation $f(\vz_1,\vz_2)$ for mutual information estimation method in the literature. The last two column report values of lower bounds of bias and variance.}
\label{tab:design_choices}
\end{table}
